Symmetry-enforced agreement of Kohn--Sham and many-body Berry phases in the SSH--Hubbard chain

We study when a density-matching Kohn--Sham (KS) description can reproduce a many-body Berry phase in a correlated insulator, despite the fact that geometric phases are functionals of the wave function. Focusing on the one-dimensional SSH--Hubbard chain on a ring as a controlled interacting topological model, we introduce a $U(1)$ twist $\theta$ (flux insertion). The many-body ground state along the full twist cycle is computed by the density-matrix renormalization group (DMRG), while the onsite interaction $U$ is tuned from the noninteracting to the strong-coupling regime. At half filling in the inversion-symmetric gapped regime, our DMRG calculations show that the density remains constant within numerical accuracy over the entire $(\theta,U)$ range studied. Thus, the density has no dependence on either the flux $\theta$ or the interaction strength $U$. Accordingly, the symmetry-preserving density constraint collapses the KS reference to an SSH-type quadratic representative with $U$-independent geometric diagnostics. Nevertheless, the many-body wave function exhibits a nontrivial geometric response: the quantum metric associated with the $\theta$-parametrized ground-state manifold depends on $\theta$ at intermediate $U$ and is strongly suppressed at large $U$, consistent with the charge fluctuation freezing. Intriguingly, the KS and many-body Berry phases coincide throughout the gapped regime as $U$ is tuned from weak to strong coupling. We show that this agreement is best understood as symmetry-enforced $\mathbb{Z}_2$ sector matching, rather than as evidence that the density encodes the many-body Berry connection.

==> sections/06_summary.tex <==
% To be written
\section{Conclusion}
In this work, we introduced a twist angle $\theta$ (a $U(1)$ gauge phase) as an adiabatic parameter for a periodic one-dimensional chain described by the SSH--Hubbard model, and numerically analyzed the geometric response of the ground state using the density-matrix renormalization group (DMRG). The main observations are summarized as follows.

First, the many-body ground state $\ket{\Psi_0(\theta,U)}$ depends nontrivially on $\theta$. In particular, the overlap between neighboring ground states on a discretized twist grid $\{\theta_j\}$, $\langle \Psi_0(\theta_j)|\Psi_0(\theta_{j+1})\rangle$, deviates systematically from unity, providing direct evidence that the wave function couples to the gauge phase and is geometrically deformed. This is consistent with the fact that the many-body Berry phase defined via the Berry connection is intrinsically determined by wave-function information.

Second, despite this wave-function-level $\theta$ dependence, the local particle density $n_i(\theta,U)$ is, within numerical accuracy, nearly independent of $\theta$ over a wide range of $U$. Therefore, the density does not directly carry information on the gauge (Berry) connection. This contrast clarifies that, in the present problem, geometric information is not transferred to local diagonal observables.

Third, by comparing the many-body Berry phase with the single-particle Berry phase obtained from a Kohn--Sham (KS) noninteracting system that reproduces the same density, we showed that the two Berry phases coincide independently of the interaction strength $U$ as long as inversion symmetry and a finite gap are maintained. In the parameter regime studied here, the KS potential constructed from the density constraint becomes effectively trivial, while the Berry phase is constrained by $\mathbb{Z}_2$ quantization; consequently, the final phase value is fixed to the same topological sector as that of the exact interacting system. Hence, the agreement of the Berry phases in the KS description should be understood not as a consequence of the density encoding geometric information, but as a consequence of the quantization constraint enforced by symmetry and the gapped structure.

As a future direction, it is important to lift the symmetry protection responsible for the $\mathbb{Z}_2$ quantization and to test whether a density-based KS construction can still reproduce the Berry phase in situations where the density response to the twist angle $\theta$ becomes nontrivial. For example, introducing an external potential that explicitly breaks spatial inversion symmetry generally removes the quantization of the Berry phase and allows it to take continuous values. In such a setting, it will be necessary to quantify to what extent a KS system constrained to reproduce the density can retain information on the many-body Berry connection. This direction will enable a quantitative assessment of how strongly the reproducibility of topological quantities within density functional theory relies on symmetry constraints, thereby clarifying the applicability and limitations of the KS framework for strongly correlated topological systems.


